Benchmarking local motion planners for navigation of mobile manipulators

There are various trajectory planners for mobile manipulators. It is often challenging to compare their performance under similar circumstances due to differences in hardware, dissimilarity of tasks and objectives, as well as uncertainties in measurements and operating environments. In this paper, we propose a simulation framework to evaluate the performance of the local trajectory planners to generate smooth, and dynamically and kinematically feasible trajectories for mobile manipulators in the same environment. We focus on local planners as they are key components that provide smooth trajectories while carrying a load, react to dynamic obstacles, and avoid collisions. We evaluate two prominent local trajectory planners, Dynamic-Window Approach (DWA) and Time Elastic Band (TEB) using the metrics that we introduce. Moreover, our software solution is applicable to any other local planners used in the Robot Operating System (ROS) framework, without additional programming effort.

==> Section_II_-_PROBLEM_STATEMENT.tex <==
\label{section:problemStatement}

As seen in section \ref{section:relatedWork}, there have been many benchmarks and evaluations on local planners for the use of mobile robots. They help with finding optimal algorithm for a given purpose that the mobile robot would be used for. The focus for this paper would be on the performance of local planners for the specific use cases of a mobile manipulator rather than a more simple mobile robot. With the added complexity of the arm attached to the base, there are more components and aspects that the local planner would have to compensate for and keep track of. One of these, which is the main focus of the paper, is how effectively the mobile manipulator will be able to carry loads using its end-effector when traversing along a planned path from the aforementioned global planner.

%The focus of this paper is different from the usual benchmarks for local planners. While most benchmarks focus on either computation time needed, travel time, or obstacle avoidance capabilities of a mobile base, these results can be further expanded by considering difference applications of mobile bases. One of these cases is mobile manipulators, generally larger than the small mobile bases used for benchmarks, which are used for pick-and-place or transportation tasks in different environments.

As the safe transportation of objects is crucial for successful operations of the mobile manipulator, it is important to make sure that the end-effector is stable so as to not impose added difficulties for when transporting the items. This means that when a grasp of an object is successful, it is best that the end-effector and arm stays stable when the mobile base is moving to another area to finish the task given. As many loads can be heavy, or quite sensitive, any small perturbation in its movement can lead to significant consequences during regular use of the mobile manipulators. Consequences can range from power losses due to the robot having to compensate for these perturbations, or, in more extreme scenarios, damage caused to the load being transported.

In most applications of mobile manipulators, high-end robots would be used so as to have high reliability and accuracy in the robot's performance. The ability of the robot to transport a load can be subject to more unreliability due to the poor performance of the local planner, rendering much of economic costs put into the robot to be wasted if the local planner is not improved. To mitigate that, our presented benchmark can help in finding planners that are optimal for this use case and which can be more simply modified to test on different robots and different local planners not covered in this paper.

%Finding out the stability of local planners in this context would allow for more research for less constrained designs for mobile manipulators as they would be able to transport more sensitive material than before without having to store it somewhere on itself before moving (like on top of the base). 

% Describe how the robot only uses a laser scanner to avoid obstacles and as input to the local planner.

==> Section_II_-_RELATED_WORKS.tex <==
\label{section:relatedWork}

A few benchmarking studies specifically focus on the ROS implementation of DWB or TEB. In \cite{pittner_systematic_2018} and \cite{cybulski_accuracy_2019}, the motion planning algorithms line DWB, TEB, and E-band are tested using small mobile robots both in simulation and in experiments. The work showed that DWB performs the fastest, and E-band is the most accurate local planner in the performed experiments. At the same time, TEB plans motions that lead the robot to the goal slightly faster than the other two algorithms. The authors also report that TEB would react the fastest to dynamic obstacles while DWB sometimes stopped to calculate its next route. In \cite{marin-plaza_global_2018, naotunna_comparison_2020} similar results are reported with a heavy, differential-driven robot carrying a Baxter manipulator. These researches confirm that TEB performs better than any of the studied algorithms at obstacle avoidance by simulating and then implementing TEB on an autonomous vehicle driving around in the real world. 

In order to improve navigation benchmarking efforts, \cite{hsieh_experimental_2016} and \cite{wen_mrpb_2021} propose two different standards. \cite{hsieh_experimental_2016} introduce the standard of worlds with different types of obstacles such as dynamic or moving. They have also proposed adding chaos in how the dynamic obstacles are set up (as in neat compared to a messy environment) and tested in real life and simulations. On the other hand, in \cite{wen_mrpb_2021} provides some standard worlds/environments to use but puts more focus on standard metrics that can be useful when running navigation benchmarks.

%There have been many papers on the smoothness of the generated path with a local planner. 
In \cite{wen_mrpb_2021} the authors have found that TEB generates much smoother paths when using a metric introduced in their research, where they would sum up the difference between two position measurements taken when the mobile base is travelling along a path. 
%The metric that they used is the size of the vectors that connect two measurements, i.e., $\sum_{i=2}^N \vert\vert\Delta\mathbf{x}_{i+1} - \Delta\mathbf{x}_{i}\vert\vert^2$. We have examined the variable descriptions in Section \ref{section:method}-\ref{subsection:path_smoothness}). %Our finding indicates that 
However, while the distance between two measurements might be minimal, this method may fail in discerning how smooth the generated path is. This metric would more accurately measure the resolution of the path rather than its smoothness. In \cite{guillen_ruiz_measuring_2020} the authors also simulate a mobile robot in different scenarios to measure the generated path's smoothness. The interesting approach they have taken is to survey the vehicle's passengers on the smoothness of their ride in the vehicle. 

Differently from the aforementioned approaches, we propose a framework to evaluate the performance of the local trajectory planners to generate smooth, and feasible trajectories for mobile manipulators, in addition to the other metrics mentioned by the previous approaches. We examine two prominent local trajectory planners, Dynamic-Window Approach (DWB) and Time Elastic Band (TEB). The software we built can be easily used for any other local planners that are available in ROS as well as other robots with minimal changes needed.
